Space-time POD-Galerkin approach for parametric flow control

In this contribution we propose reduced order methods to fast and reliably solve parametrized optimal control problems governed by time dependent nonlinear partial differential equations. Our goal is to provide a tool to deal with the time evolution of several nonlinear optimality systems in many-query context, where a system must be analysed for various physical and geometrical features. Optimal control can be used in order to fill the gap between collected data and mathematical model and it is usually related to very time consuming activities: inverse problems, statistics, etc. Standard discretization techniques may lead to unbearable simulations for real applications. We aim at showing how reduced order modelling can solve this issue. We rely on a space-time POD-Galerkin reduction in order to solve the optimal control problem in a low dimensional reduced space in a fast way for several parametric instances. The proposed algorithm is validated with a numerical test based on environmental sciences: a reduced optimal control problem governed by viscous Shallow Waters Equations parametrized not only in the physics features, but also in the geometrical ones. We will show how the reduced model can be useful in order to recover desired velocity and height profiles more rapidly with respect to the standard simulation, not losing accuracy.

==> intro.tex <==

Parametrized optimal control problems (\ocp s) governed by parametrized partial differential equations (PDE($\boldsymbol{\mu}$)s) are very powerful mathematical formulations, to be exploited in several applications in different scientific fields, see \cite{leugering2014trends} for an overview. Among the possible impact that \ocp s  can have in scientific research, we will refer to the investigation into problems dealing with environmental sciences applications. Indeed, this work is motivated by the ongoing demand for reaching fast and accurate simulations for the coastal marine environment safeguard. The marine ecosystem is linked to other important social factors such as, for example, economic growth, natural resources preservation, monitoring plans. 
 Furthermore, the marine environment is very far to be completely understood, since it is linked to very complicated natural phenomena and anthropic consequences \cite{cavallini2012quasi, mosetti2005innovative, golfo}.\\
For sure, the parametric setting is necessary in order to study different configurations: the parameter $\boldsymbol{\mu} \in \Cal P \subset \mathbb R^d$ could represent a variety of physical phenomena. Moreover, in the environmental field, the theory of \ocp s fits well with the need of increasing the models forecast capabilities through a data assimilation approach \cite{ghil1991data,kalnay2003atmospheric,tziperman1989optimal}. A lot of effort is made in order to make PDEs models based predictions the most similar to collected data. 
Data assimilation \ocp s have been already analysed in several works, as \cite{phd, quarteroni2005numerical, quarteroni2007reduced, Strazzullo1, ZakiaMaria}. \fb{Yet, }the main drawback of data assimilated problems is the huge computational complexity which still limits their applicability, most of all if the optimization problem deals with very complicated parametric flow models, as the ones used in marine and coastal engineering. Furthermore, in the \fb{described context}, accurate simulations are required in a small amount of time, in order to better study and analyse them: indeed, the primal goal is to manage different situations. This is the reason \fb{that motivates 
the use of Reduced Order Methods (ROMs)} as a suitable approach for rapid and accurate surrogate simulations of partial differential equations PDE($\boldsymbol{\mu}$)s \cite{hesthaven2015certified, prud2002reliable, RozzaHuynhPatera2008}. The main feature of ROM techniques is to solve the parametrized problem in a low dimensional framework in order to save computational resources which can be exploited for the analysis of several parametric configurations: ROMs recast a time consuming simulation, the \emph{truth problem}, into a new fast and reliable formulation thanks to a Galerkin projection into reduced spaces, generated by basis functions derived from a proper orthogonal decomposition (POD) algorithm, as presented in \cite{ballarin2015supremizer, burkardt2006pod, Chapelle2013, hesthaven2015certified}.\\
In general, reduction methods for parametrized nonlinear time dependent \ocp s are very complex to analyse both theoretically and numerically. Although the literature is quite consolidated for steady constraints, see for example \cite{bader2016certified,bader2015certified,dede2010reduced, gerner2012certified,karcher2014certified,karcher2018certified,kunisch2008proper,negri2013reduced,negri2015reduced,quarteroni2007reduced},  \fb{where} the interested reader may find theoretical and numerical analysis for different linear models, there is very small knowledge about time dependency \cite{Iapichino2, karcher_grepl_2014, Strazzullo1,ZakiaMaria}. Another difficulty to be overcome is the treatment and the reduction of nonlinear \ocp s, see for example 
\cite{LassilaManzoniQuarteroniRozza2013a, rozza2012reduction, Strazzullo1,ZakiaMaria,Zakia}. 
\\In this work, we focus on ROM for \ocp s with quadratic cost functional constrained to parametrized Shallow Waters Equations (SWEs). The latter is a very useful model in environmental sciences, which is capable to simulate various marine phenomena such as, for example, tidal flows and mixing, currents action on shores and coasts, planetary flows and even tsunamis \cite{cavallini2012quasi,Shallow}. The state equation proposed is nonlinear and time dependent: this leads to growing complexity in the \fb{solution} of the optimality system in a real-time context. Indeed, even if the state equation and the control problem have been analysed and managed numerically with many approaches, see for example \cite{agoshkov1994recent2,  Agoshkov1993, agoshkov1994recent, agoshkov2007optimal, ferrari2004new, miglio1999finite, miglio2005model, miglio2005model2, ricchiuto2007application, ricchiuto2009stabilized,  takase2010space}, their parametric formulation is still quite unexplored and based on time reduction of the state equation \cite{Navon2, Navon1}.
\\ The main novelty of this work is to perform reduction on the parametric space on the complete SWEs model, i.e nonlinear and time dependent, in a solution tracking optimal control framework.
We aim at making a further step towards forecasting data assimilated coastal models which could be used as resources to manage realistic experiments involved in marine sciences with environmental prevision purposes. 
Indeed, ROMs could be very effective in providing a large number of parametric simulations in an acceptable amount of time, and this can be very useful in order to understand better the \fb{considered physical phenomenon}.
Morever, we extend the standard reduced techniques for \ocp s, already exploited for steady and time dependent linear problems, in order to deal with nonlinear state equations.
We will show how ROM could be a good strategy which will give us faster, but still accurate, results.

\no The work is outlined as follows. In Section 2, we first present the SWEs model and then we show it in the optimal control framework. Moreover, we briefly describe the Finite Element approximation and the algebraic version of the presented solution tracking problem. Section 3 will introduce the basic ideas behind ROM discretization for \ocp s \cite{hesthaven2015certified, ito1998reduced, karcher2014certified}: we will describe POD sampling algorithm for \ocp s and the aggregated reduced spaces technique used in \cite{dede2010reduced, negri2015reduced,negri2013reduced} which will guarantee the solvability of the optimality system in its saddle point formulation. Moreover, we will briefly mention affine decomposition assumption, see e.g. \cite{hesthaven2015certified}, needed for an efficient \fb{solve} of the reduced system. In Section 4, we test our methodology on a parametrized \ocp s governed by the SWE equations, inspired by an uncontrolled numerical test case of \cite{ferrari2004new}, where the evolution a Gaussian water height is studied. Our test case aims at recovering a given desired velocity-height profile. Finally, conclusions and perspectives follow in Section 5.

